MOTOR: A Time-To-Event Foundation Model For Structured Medical Records

We present a self-supervised, time-to-event (TTE) foundation model called MOTOR (Many Outcome Time Oriented Representations) which is pretrained on timestamped sequences of events in electronic health records (EHR) and health insurance claims. TTE models are used for estimating the probability distribution of the time until a specific event occurs, which is an important task in medical settings. TTE models provide many advantages over classification using fixed time horizons, including naturally handling censored observations, but are challenging to train with limited labeled data. MOTOR addresses this challenge by pretraining on up to 55M patient records (9B clinical events). We evaluate MOTOR's transfer learning performance on 19 tasks, across 3 patient databases (a private EHR system, MIMIC-IV, and Merative claims data). Task-specific models adapted from MOTOR improve time-dependent C statistics by 4.6% over state-of-the-art, improve label efficiency by up to 95% ,and are more robust to temporal distributional shifts. We further evaluate cross-site portability by adapting our MOTOR foundation model for six prediction tasks on the MIMIC-IV dataset, where it outperforms all baselines. MOTOR is the first foundation model for medical TTE predictions and we release a 143M parameter pretrained model for research use at [redacted URL].

==> Tables/finetuning_ablation.tex <==
\begin{table}[ht]
\centering
\caption{Impact of sample sizes for fine-tuning MOTOR on the time-dependent C statistic. We utilize a subset of the full training data to conduct fine-tuning. 100\% indicates the entire training dataset.}
\vspace{2pt}
\label{t:finetune}
\begin{tabular}{lcccccc}
  \toprule
        \% Used  & Celiac &  Heart Attack & Lupus & NAFLD & Pancretic Cancer & Stroke  \\\midrule
5\% & 0.785 & 0.878 & 0.840 & 0.851 & 0.849 & 0.868\\%\hline
10\% & 0.781 & 0.874 & 0.844 & 0.854 & 0.854 & 0.868\\%\hline
25\% & 0.790 & 0.880 & 0.845 & 0.856 & 0.859 & 0.869\\%\hline
100\% & \textbf{0.802} & \textbf{0.884} & \textbf{0.850} & \textbf{0.859} & \textbf{0.865} & \textbf{0.874}\\\bottomrule




\end{tabular}
\end{table}

==> Tables/finetuning_ablation_delta.tex <==
\begin{table}[ht]
\centering
\caption{95\% confidence intervals for the difference in time-dependent C statistic between fine-tuning on 100\% of the training data vs subsets of the data. $\ast$ indicate statistically significant entries at p = 0.05. }
\vspace{2pt}
\label{t:finetune_delta}
\resizebox{\textwidth}{!}{\begin{tabular}{lcccccc}
  \toprule
        \% Used  & Celiac &  Heart Attack & Lupus & NAFLD & Pancretic Cancer & Stroke  \\\midrule
5\% & [-0.029, -0.005]\text{*}  & [-0.010, -0.001]\text{*}  & [-0.018, -0.003]\text{*}  & [-0.010, -0.007]\text{*}  & [-0.025, -0.004]\text{*}  & [-0.009, -0.004]\text{*} \\
10\% & [-0.033, -0.008]\text{*}  & [-0.015, -0.004]\text{*}  & [-0.012, 0.000] & [-0.006, -0.004]\text{*}  & [-0.018, -0.003]\text{*}  & [-0.008, -0.004]\text{*} \\
25\% & [-0.018, -0.005]\text{*}  & [-0.007, -0.000]\text{*}  & [-0.010, 0.000] & [-0.005, -0.003]\text{*}  & [-0.010, -0.002]\text{*}  & [-0.006, -0.004]\text{*} \\
100\% & [0.000, 0.000] & [0.000, 0.000] & [0.000, 0.000] & [0.000, 0.000] & [0.000, 0.000] & [0.000, 0.000]\\\bottomrule




\end{tabular}}
\end{table}

==> Tables/mimic_confidence.tex <==
\begin{table}[ht]
\centering
\caption{95\% confidence intervals of difference in time-dependent C statistic between MOTOR-Transfer Probe and the other methods. Higher numbers are considered better for this metric.  $\ast$ indicates statistically significant entries at p = 0.05.}
\vspace{2pt}
\label{t:mimic_confidence}
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccc}
  \toprule
        Method  & Celiac &  Heart Attack & Lupus & NAFLD & Pancretic Cancer & Stroke  \\\midrule
        \multicolumn{7}{c}{EHR-OMOP}  \\\midrule
Cox PH & [-0.140, -0.088]\text{*}  & [-0.146, -0.105]\text{*}  & [-0.113, -0.073]\text{*}  & [-0.147, -0.129]\text{*}  & [-0.093, -0.050]\text{*}  & [-0.105, -0.086]\text{*} \\
DeepSurv & [-0.120, -0.076]\text{*}  & [-0.079, -0.048]\text{*}  & [-0.091, -0.056]\text{*}  & [-0.070, -0.057]\text{*}  & [-0.075, -0.035]\text{*}  & [-0.052, -0.037]\text{*} \\
DSM & [-0.115, -0.075]\text{*}  & [-0.076, -0.043]\text{*}  & [-0.097, -0.060]\text{*}  & [-0.065, -0.054]\text{*}  & [-0.078, -0.035]\text{*}  & [-0.047, -0.034]\text{*} \\
DeepHit & [-0.132, -0.084]\text{*}  & [-0.078, -0.043]\text{*}  & [-0.074, -0.038]\text{*}  & [-0.065, -0.052]\text{*}  & [-0.079, -0.037]\text{*}  & [-0.049, -0.035]\text{*} \\
RSF & [-0.096, -0.051]\text{*}  & [-0.067, -0.036]\text{*}  & [-0.094, -0.057]\text{*}  & [-0.068, -0.055]\text{*}  & [-0.060, -0.023]\text{*}  & [-0.041, -0.027]\text{*} \\
MOTOR-Scratch & [-0.131, -0.083]\text{*}  & [-0.114, -0.073]\text{*}  & [-0.081, -0.041]\text{*}  & [-0.047, -0.037]\text{*}  & [-0.114, -0.064]\text{*}  & [-0.050, -0.036]\text{*} \\
MOTOR-Probe & [-0.010, 0.009] & [-0.008, 0.001] & [-0.020, -0.005]\text{*}  & [-0.008, -0.002]\text{*}  & [-0.006, 0.004] & [-0.004, 0.003]\\
MOTOR-Finetune & [0.000, 0.000] & [0.000, 0.000] & [0.000, 0.000] & [0.000, 0.000] & [0.000, 0.000] & [0.000, 0.000]\\
\midrule
        \multicolumn{7}{c}{MERATIVE}   \\\midrule
Cox PH & [-0.273, -0.251]\text{*}  & [-0.051, -0.043]\text{*}  & [-0.095, -0.085]\text{*}  & [-0.069, -0.056]\text{*}  & [-0.219, -0.203]\text{*}  & [-0.107, -0.096]\text{*} \\
DeepSurv & [-0.048, -0.037]\text{*}  & [-0.019, -0.013]\text{*}  & [-0.034, -0.028]\text{*}  & [-0.039, -0.028]\text{*}  & [-0.036, -0.029]\text{*}  & [-0.046, -0.038]\text{*} \\
DSM & [-0.041, -0.031]\text{*}  & [-0.020, -0.015]\text{*}  & [-0.029, -0.023]\text{*}  & [-0.034, -0.024]\text{*}  & [-0.033, -0.027]\text{*}  & [-0.040, -0.032]\text{*} \\
DeepHit & [-0.045, -0.034]\text{*}  & [-0.018, -0.014]\text{*}  & [-0.032, -0.026]\text{*}  & [-0.039, -0.028]\text{*}  & [-0.036, -0.030]\text{*}  & [-0.045, -0.036]\text{*} \\
RSF & [-0.062, -0.052]\text{*}  & [-0.022, -0.017]\text{*}  & [-0.037, -0.031]\text{*}  & [-0.028, -0.019]\text{*}  & [-0.039, -0.032]\text{*}  & [-0.053, -0.045]\text{*} \\
MOTOR-Scratch & [-0.029, -0.021]\text{*}  & [-0.011, -0.006]\text{*}  & [-0.015, -0.011]\text{*}  & [-0.015, -0.008]\text{*}  & [-0.015, -0.010]\text{*}  & [-0.023, -0.017]\text{*} \\
MOTOR-Probe & [-0.010, -0.004]\text{*}  & [-0.003, 0.000] & [-0.008, -0.004]\text{*}  & [-0.008, -0.002]\text{*}  & [-0.011, -0.007]\text{*}  & [-0.008, -0.004]\text{*} \\
MOTOR-Finetune & [0.000, 0.000] & [0.000, 0.000] & [0.000, 0.000] & [0.000, 0.000] & [0.000, 0.000] & [0.000, 0.000]\\

\bottomrule

\end{tabular}}
\end{table}

==> Tables/mimic_light.tex <==
\begin{table}[ht]
\centering
\caption{Time-dependent C statistic for MOTOR-Transfer Probe and the best baseline for the code-based tasks on MIMIC-IV. Bolding indicates the best performing model. }
\vspace{2pt}
\label{t:mimic_light}
\begin{tabular}{lcccccccc}
  \toprule
        Method  & Celiac &  HA & Lupus & NAFLD & Cancer & Stroke  \\\midrule
%  EHR-OMOP \\
%  \midrule
Strongest Baseline & 0.625 & 0.820 & 0.807 & 0.736 & 0.748 & 0.780\\
MOTOR-Transfer Probe &  \textbf{0.628} & \textbf{0.850} & \textbf{0.819} & \textbf{0.802} & \textbf{0.828} & \textbf{0.812}\\ 
\bottomrule
\end{tabular}
\end{table}


==> Tables/pretraining_ablation.tex <==
\begin{table}[ht]
\centering
\caption{Impact of pretraining on the performance of MOTOR in terms of the time-dependent C statistic on the code-based tasks. We utilize a subset of the full training data to conduct pretraining. K (thousand), M (million).}
\vspace{2pt}
\label{t:pretrain}
\begin{tabular}{lcccccc}
  \toprule
         \# Patients For Pretraining & Celiac &  Heart Attack & Lupus & NAFLD & Pancretic Cancer & Stroke  \\\midrule
95K (5\%) & 0.694 & 0.843 & 0.740 & 0.768 & 0.825 & 0.824\\%\hline
191K (10\%) & 0.714 & 0.849 & 0.749 & 0.786 & 0.831 & 0.828\\%\hline
478K (25\%) & 0.742 & 0.853 & 0.788 & 0.799 & 0.837 & 0.833\\%\hline
1.91M (100\%) & \textbf{0.802} & \textbf{0.884} & \textbf{0.850} & \textbf{0.859} & \textbf{0.865} & \textbf{0.874}\\\bottomrule
\end{tabular}
\end{table}

==> Tables/pretraining_ablation_delta.tex <==
\begin{table}[ht]
\centering
\caption{95\% confidence intervals for the difference in time-dependent C statistic between pretraining on 100\% of the training data vs more limited subsets. $\ast$ indicates statistically significant entries at p = 0.05.}
\vspace{2pt}
\label{t:pretrain_delta}
\resizebox{\textwidth}{!}{\begin{tabular}{lcccccc}
  \toprule
         \% Used & Celiac &  Heart Attack & Lupus & NAFLD & Pancretic Cancer & Stroke  \\\midrule
5\% & [-0.130, -0.084]\text{*}  & [-0.052, -0.028]\text{*}  & [-0.132, -0.089]\text{*}  & [-0.099, -0.084]\text{*}  & [-0.058, -0.022]\text{*}  & [-0.057, -0.044]\text{*} \\
10\% & [-0.109, -0.066]\text{*}  & [-0.046, -0.023]\text{*}  & [-0.124, -0.081]\text{*}  & [-0.080, -0.067]\text{*}  & [-0.052, -0.016]\text{*}  & [-0.053, -0.040]\text{*} \\
25\% & [-0.078, -0.041]\text{*}  & [-0.041, -0.020]\text{*}  & [-0.081, -0.044]\text{*}  & [-0.066, -0.054]\text{*}  & [-0.041, -0.014]\text{*}  & [-0.047, -0.035]\text{*} \\
100\% & [0.000, 0.000] & [0.000, 0.000] & [0.000, 0.000] & [0.000, 0.000] & [0.000, 0.000] & [0.000, 0.000]\\\bottomrule


\end{tabular}}
\end{table}

==> Tables/prospective_light.tex <==

\begin{table}[ht]
\centering
\caption{Time-dependent C statistic for the best MOTOR model and the best baseline for the code-based tasks on a prospective 9-month EHR-OMOP dataset. Bolding indicates the best performing model. }
\vspace{2pt}
\label{t:prospective_light}
\begin{tabular}{lcccccccc}
  \toprule
        Method  & Celiac &  HA & Lupus & NAFLD & Cancer & Stroke  \\\midrule
%  EHR-OMOP \\
%  \midrule
Strongest Baseline & 0.682 & 0.776 & 0.810 & 0.750 & 0.786 & 0.768 \\ 
Strongest MOTOR   & \textbf{0.792}&\textbf{0.843}&\textbf{0.880}&\textbf{0.809} &	\textbf{0.870}&	\textbf{0.836}\\
\midrule

\end{tabular}
\end{table}


==> Tables/timing_experiments.tex <==
\begin{table}[ht]
\centering
\caption{The time it takes to train a target task model, in minutes. Each run is given 16 CPU cores, one V100 GPU, and 100 GB of RAM. The fastest method for each target task is bolded.}
\vspace{2pt}
\label{t:timing}
\begin{tabular}{lccccccc}
  \toprule
        Method  & Celiac &  Heart Attack & Lupus & NAFLD & Pancretic Cancer & Stroke  \\\midrule
RSF & \textbf{1.82} & \textbf{1.21} & 5.80 & 93.31 & \textbf{2.08} & 22.22 \\
MOTOR & 2.35 & 2.47 & \textbf{2.40} & \textbf{11.45} & 2.16 & \textbf{7.50} \\ \bottomrule




\end{tabular}
\end{table}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

